Enhancement of Double-Close-Binary Quadruples

Double-close-binary quadruples (2+2 systems) are hierarchical systems of four stars where two short-period binary systems move around their common center of mass on a wider orbit. Using Gaia Early Data Release 3, we search for comoving pairs where both components are eclipsing binaries. We present eight 2+2 quadruple systems with inner orbital periods of $<$ 0.4 days and with outer separations of $\gtrsim 1000$ AU. All but one system are newly discovered by this work, and we catalog their orbital information measured from their light curves. We find that the occurrence rate of 2+2 quadruples is 7.3 $\pm$ 2.6 times higher than what is expected from random pairings of field stars. At most a factor of $\sim$2 enhancement may be explained by the age and metallicity dependence of the eclipsing binary fraction in the field stellar population. The remaining factor of $\sim$3 represents a genuine enhancement of the production of short-period binaries in wide-separation ($>10^3$ AU) pairs, suggesting a close binary formation channel that may be enhanced by the presence of wide companions.

==> addons.tex <==
    Double-close-binary quadruple systems are of interest as they present a way to observe the dynamics of high-order stellar systems. Not only would understanding of quadruple dynamics give insight into how high order systems form and behave, but could also provide important information in other areas of study like star formation.
    If the dynamics of quadruple systems are responsible for shrinking the periods of the inner binary pairs towards contact, then it would be expected that the probability of a binary's companion being another  binary would be enhanced when compared to the probability of a field star being an eclipsing binary. Enhancement would indicate that EBs are more likely to have been formed by a quadruple system than to have been formed on their own, suggesting that the astrophysical dynamics at play in quadruple systems might favorably create EBs. We search for this enhancement using Gaia EDR3 astrometric data. By identifying the number of comoving pairs of variable stars in the catalog, the probability of an EB's wide companion being another EB can be estimated. To calculate the enhancement of this value, we can compare this to the reported probability of a field star being an EB. In this study we specifically search for optically resolvable, and therefore wide-separation, 2+2 systems. With such a large outer orbit, dynamic interactions would likely    
    
Superficial cuts are later imposed to create the parent sample, but a large initial query allows for greater freedom in cuts later. Imposing further cuts  will be done to limit flaring stars that would contaminate the variable sample and stars that are too far away or dim to have reliable astrometry. 

% \begin{table*}[]
% 	\centering
% 	\caption{Catalog for 5\% 2+2 systems.}
% 	\label{tab:catalog}
% 	\begin{tabular}{lllllllllll} 
% 		\hline \hline
% 		source id 0 & ra0 & dec0 & source id 1 & ra1 & dec1 & separation (AU) & Period0 & Period1 & survey \\
% 		\hline
% 		3190750999704606464 & 0 & 0 & 3190750999704606464 & 0 & 0  \\
% 		3190750999704606464 & 0 & 0 & 3190750999704606464 & 0 & 0  \\
% 		\hline
		
% 		\hline \hline
% 	\\
% 	\end{tabular}
% \end{table*}


% \begin{table*}[]
% 	\centering
% 	\caption{Catalog for 3\% 2+2 systems.}
% 	\label{tab:catalog}
% 	\begin{tabular}{llllllll} 
% 		\hline \hline
% 		source id 0 & ra0 & dec0 & source id 1 & ra1 & dec1 & separation (AU) \\
% 		\hline
% 		000000 & 0 & 0 & 0 & 0 & 0  \\
% 		000000 & 0 & 0 & 0 & 0 & 0  \\
% 		\hline
		
% 		\hline \hline
% 		\\
% 	\end{tabular}
% \end{table*}
    




